The Geometry of Types (Long Version)

We show that time complexity analysis of higher-order functional programs can be effectively reduced to an arguably simpler (although computationally equivalent) verification problem, namely checking first-order inequalities for validity. This is done by giving an efficient inference algorithm for linear dependent types which, given a PCF term, produces in output both a linear dependent type and a cost expression for the term, together with a set of proof obligations. Actually, the output type judgement is derivable iff all proof obligations are valid. This, coupled with the already known relative completeness of linear dependent types, ensures that no information is lost, i.e., that there are no false positives or negatives. Moreover, the procedure reflects the difficulty of the original problem: simple PCF terms give rise to sets of proof obligations which are easy to solve. The latter can then be put in a format suitable for automatic or semi-automatic verification by external solvers. Ongoing experimental evaluation has produced encouraging results, which are briefly presented in the paper.

==> sauve_4.tex <==
\section{Relative Type Inference}
\label{sec:typeinf}
Given on the one hand soundness and relative completeness of \dlpcf, and on the other
undecidability of complexity analysis for \PCF\ programs, one may wonder
whether looking for a type inference procedure makes sense at all. As stressed in the
Introduction, however, we will not give a type inference algorithm \emph{per se}, but
rather reduce type inference to the problem of checking a set of inequalities modulo
an equational program (see Figure~\ref{fig:context}). This is the reason why we can only
claim type inference can be solved in a \emph{relative} sense, i.e. assuming an oracle
for proof obligations exists. 

Why is solving relative type inference useful? Suppose you have a program $\t:\NatPCF\toPCF\NatPCF$
and you want to prove that it works in a number of steps bounded by a polynomial
$p:\int\rightarrow\int$ (\eg, $p(x)=4\cdot x+7$). You can of course proceed by building a \dlpcf\ type
derivation for $\t$ by hand, or even reasoning directly on the complexity of $\t$. Relative type
inference simplifies your life: it outputs an equational program $\ep$, a \emph{precise} type derivation
for $\t$ whose conclusion is $a;;\vdash^\ep_\I \t:\NatU{a}\marr{1}\NatU{\J}$ and a set $\mathcal{I}$ of 
inequalities on the same signature as the one of $\ep$. Your original problem, then, is reduced to verifing 
$\models^\ep\mathcal{I}\cup\{\I\leq p(a)\}$. This is arguably a problem which is easier to be solved
in practice than the original one: first of all, it is not complexity analysis but rather a problem
about the value of arithmetical expressions, secondly it only deals with first-order objects.

\subsection{An Informal Account}
From the brief discussion in Section~\ref{sec:informal}, it should be clear that devising a 
compositional type inference procedure for \dlpcf\ is nontrivial: the type one assigns to a subterm
heavily depends on the ways the rest of the program uses the subterm. The solution we
adopt is here consists in allowing the algorithm to return \emph{partially unspecified} equational programs:
$\ep$ as produced in output by $\mathcal{T}$ gives meaning to all the symbols in
the output type derivation \emph{except} those occurring in negative position in its conclusion.

To better understand how the type inference algorithm works, let us consider the following term $\t$:
$$
\u\v=(`lx.`ly.x(xy))(`lz.\suc(z)).
$$
The subterm $\u$ can be given type $(\NatPCF\toPCF\NatPCF)\toPCF\NatPCF\toPCF\NatPCF$ in \PCF, while
$\v$ has type $\NatPCF\toPCF\NatPCF$. This means $\t$ as a whole is a first-order function.
The type inference algorithm proceeds by giving types to $\u$ and
to $\v$ separately, then assembling the two into one. Suppose we start with $\v$. The type inference
algorithm refines $\NatPCF\toPCF\NatPCF$ into $`s=\NatU{f(a,b)}\marr{b<h(a)}\NatU{g(a,b)}$ and the
equational program $\ep_\v$, which gives meaning to $f$ in terms of $g$:
\begin{align*}
g(a,b)&=f(a,b)+1
\end{align*}
Observe how both $f$ and $h$ are not specifed in $\ep_\v$, because they appear in \emph{negative} position in $`s$:
$f(a,b)$ intuitively corresponds the argument(s) $\v$ will be applied to, while $\h(a)$ is the number of times
$\v$ will be used. Notice that everything is parametrized on $a$, which is something like a global parameter
that will later be set as the input to $\t$. The function $\u$, on the other hand, is given type
$$
\begin{array}{c}
(\NatU{p(a,b,c)}\marr{c<j(a,b)}\NatU{q(a,b,c)})\\
\marr{b<k(a)}\\
\NatU{r(a,b,c)}\marr{c<m(a,b)}\NatU{s(a,b,c)}
\end{array}
$$
The newly introduced function symbol are subject to the following equations:
\begin{align*}
j(a,b)&=2\cdot m(a,b)\\
s(a,b,c)&=q(a,b,2c)\\
p(a,b,2c)&=q(a,b,2c+1)\\
p(a,b,2c+1)&=r(a,b,2c)
\end{align*}
Again, notice that some functions are left unspecified, namely $r$, $m$ and $q$.
Now, a type for $\u\v$ can be found by just combining the types for $\u$ and $\v$,
somehow following the typing rule for applications. First of all, the number of times
$\u$ needs to be copied is set to $1$ by the equation $k(a)=1$. Then, the matching
symbols of $\u$ and $\v$ are defined one in terms of the others:
\begin{align*}
q(a,0,b)&=g(a,b)\\
f(a,b)&=p(a,0,b)\\
h(a)&=j(a,0)
\end{align*}
This is the last step of type inference, so it is safe to stipulate that
$m(a,0)=1$ and that $r(a,0,c)=a$, thus obtaining a fully specified equational
program $\ep$ and the following type $`t$ for $\t$:
$$
\NatU{a}\marr{c<1}\NatU{s(a,0,c)}.
$$
As an exercise, the reader can verify that the equational program above allows to
verify that $s(a,0,0)=a+2$, and that 
$$
\judg{a}{\emptyset}{\emptyset}{2}{\t}{`t}.
$$


\subsection{The Main Algorithm}

\subsubsection{Eliminating subsumption rule}
\label{sec:elim-subs}

The general algorithm has a \PCF\ term~\terme\ in input, and returns a typing derivation~\der\ for~\terme, together with an equational program~\ep\ and a set of so-called \emph{side conditions}~\scond.
As we mentioned in at the end of Section~\ref{sec:typing}, the typing judgement returned for~\terme\ (in the conclusion of~\der) is \emph{precise}, in the sense that all occurences of the basic type \Nat{\I}{\J} are in fact of the form \NatU{\I}, and that the cost and all potentials~\H\ appearing in a subtype \mtyp{\H}{\A} are kept as low as possible.
Concretely , it means that the subsumption rule is restricted to
\begin{displaymath}
  \frac{\judg{\fiv}{\ictx}{`G}{\I}{t}{`s}
    \qquad
    \begin{array}[b]{r@{~}l@{\,}l}
      \sjudg{\fiv}{\ictx&}{`D&`=`G}
      \\
      \sjudg{\fiv}{\ictx&}{`s&`=`t}
      \\
      \ijudg{\fiv}{\ictx&}{\I&=\J}
    \end{array}
  }{\judg{\fiv}{\ictx}{`D}{\J}{t}{`t}}
\end{displaymath}
In such a rule, assuming that types~$`s$ and~$`t$ have the same \PCF\ skeleton, as well as both contexts~$`D$ and~$`G$, the three premisses on the right come down to a set of semantic judgments on the form
$\big\{\ijudg{\fiv}{\ictx}{\K_i=\H_i}\big\}$ 
(see Figure~\ref{fig:tsub})
where the $\K_i$'s are indexes appearing in~$`s$ or~$`D$ (or \I\ itself) and the $\H_i$'s appear in~$`t$ or~$`G$ (or is~\J).
If moreover, for each of these semantic judgements, the equality $\K_i=\H_i$ is present in~\ep, then the three premisses  on the right are equivalent to the conjunction (on~$i$) of all the properties
\begin{center}
  ``\itp{\H_i} is defined for any $`r:\fiv→\int$ satisfying \ictx''
\end{center}
(\cf\ Section~\ref{sec:sem-judg}), that we write \ijudg{\fiv}{\ictx}{\H_i`|}.
Actually the typing derivation~\der\ returned by the algorithm corresponds to a \dlpcfv\ derivation for~\terme, in which all the subsumption rules have been erased and the corresponding properties \ijudg{\fiv}{\ictx}{\H`|} have been put as side conditions in~\scond.
We call it a \emph{pseudo \dlpcfv\ typing judgement}.
It has the property that its conclusion is a derivable \dlpcf\ typing judgment for~\ep\ \textit{iff} the side conditions~\scond\ are valid.

\subsubsection{Structure of the algorithm}
\label{sec:algo-struct}

The type inference algorithm proceeds as follows:
\\
\textbf{Input:} \terme\ (\PCF \ terme)
\\
\textbf{Output:} \der\ (typing derivation)~;~
\ep\ (equational program)~;~
\scond\ (side conditions)

\begin{enumerate}
\item Compute~\derpcf, the \PCF\ type derivation of~\terme.
\item Annotate every \PCF\ type of the conclusion judgment of~\derpcf\ with fresh function symbols, to get a \dlpcfv\ typing judgment $\typjudg=\judg{∅}{∅}{`G}{}{\terme}{`t_0}$.
\item Construct recursively the equational program and the set of side conditions calling the function \mainfct\ with \typjudg, \derpcf, $\ep=∅$ and $\scond=∅$.
\item Return \der\, together with \ep\ and \scond\ as computed by \mainfct.
\end{enumerate}
A \PCF\ typing derivation the ``skeleton'' of a \dlpcf\ typing derivation (obtained by erasing all the indexes and the subsumption rules).
In \PCF\ the typing is decidable, and the first step raises no difficulty.
%The second one just requires to generate as many fresh symbol as %necessary, which can be done with a global counter (we may also need %it for the \mainfct\ function).
The core of the algorithm leads in the third step.

\subsubsection{Main recursive function}
\label{sec:main-func}

The function \mainfct\ has the following signature:
\begin{displaymath}
  \mainfct(\typjudg,\derpcf,\ep,\scond)
  \quad\mapsto\qquad
  (\der,\ep',\scond')~.
\end{displaymath}
\typjudg\ is a \dlpcfv\ typing judgment (without the cost) corresponding to the conclusion of~\derpcf, and~$\ep'$ and~$\scond'$ include~$\ep$ and~$\scond$ respectively.
\der\ is a pseudo \dlpcfv\ derivation with conclusion~\typjudg\ (with a cost).
It corresponds actually to a correct \dlpcfv\ derivation \textit{iff} all formulae in~$\scond'$ are valid.

The algorithm goes by induction on the \PCF\ typing derivation, annotates progressively \derpcf\ to turn it into a \textit{pseudo} \dlpcfv\ typing judgment, and construct the equational program and the set of side conditions.
Depending on the last typing rule used in~\derpcf, computing \mainfct(\typjudg,\derpcf,\ep,\scond) can be simple or not.
For instance, if it ends with
\vspace{-10pt}
\begin{displaymath}
  \frac{
    \begin{array}{c}
      \vdots \\
      `G_0\vdash\u:\NatPCF
    \end{array}
  }{`G_0\vdash\suc(\u):\NatPCF}
\end{displaymath}
then \typjudg\ is on the form \judg{\fiv}{\ictx}{`G}{}{\suc(\u)}{\NatU{\I}}.
In this case we just have to:
\begin{varenumerate}
\item create a fresh symbol~\J.
\item compute (by recursion) $(\der',\ep',\scond') =$\\
  \begin{math}
    \mainfct(\typjudg',\derpcf',\ep`U\{\I=\J+\one\},\scond`U\{\ijudg{\fiv}{\ictx}{\J`|}\})
  \end{math}
  where $\typjudg'=\judg{\fiv}{\ictx}{`G}{}{\u}{\NatU{\J}}$ and 
  $\derpcf'$ is the premiss of~\derpcf.
\item return $(\der,\ep',\scond')$, where 
  \begin{math}\displaystyle
    \der =
    \frac{\der'}{
      \judg{\fiv}{\ictx}{`G}{\K_{\text{cost}}}{\suc(\u)}{\NatU{\I}}
    }~,
  \end{math}
  and $\K_{\text{cost}}$ is the same as in~$\der'$.
\end{varenumerate}
\vspace{5pt}
Things get more intricate when~\derpcf\ ends using the rule (\textit{App}):
\vspace{-5pt}
\begin{displaymath}
  \frac{(d_1):
    \begin{array}[b]{c}
      \vdots \\
      `G_1\vdash\t:U\toPCF T
    \end{array}
    \qquad (d_2):
    \begin{array}[b]{c}
      \vdots \\
      `G_2\vdash\u:U
    \end{array}
  }{`G_0\vdash\t\u:T}
\end{displaymath}
In this case \typjudg\ is on the form \judg{\fiv}{\ictx}{`D}{}{\t\u}{`t_0}.
In order to call recursively \mainfct\ on~$d_1$ and~$d_2$, we need two \dlpcfv\ judgment
\begin{math}
  \typjudg_1=\judg{\fiv}{\ictx}{`D_1}{}{\t}{\arrv{\one}{`s}{`t}}
\end{math}
and
\begin{math}
  \typjudg_2=\judg{\fiv}{\ictx}{`D_2}{}{\u}{`s\isubst{\zero}}
\end{math}, and to garanty that
\begin{displaymath}
  `D`=`D_1\uplus`D_2
  \quad\text{and}\quad
  `t_0`=`t\isubst{\zero}~.
\end{displaymath}
Do do so, we create $\typjudg_1$ and $\typjudg_2$ with fresh function symbols in the type and the context, and we call auxilliary functions to build the equational program and the side conditions ensuring these type equivalence.
The auxiliary function that ensures $`D`=`D_1\uplus`D_2$ is called \emph{contraction} (which refers to contraction rule of Linear Logic: \begin{math}\displaystyle
  \frac{`G,!A,!A\vdash B}{`G,!A\vdash B}
\end{math}
)
and the one that guarentees $`t_0`=`t\isubst{\zero}$ is called \emph{dereliction} (which refers to the dereliction principle of \LL:
$!A→A$).



\subsection{Auxiliary Algorithms and Linear Logic}
The design of systems of linear dependen types such as \dlpcfv\ and \dlpcfn\ is
strongly inspired by \BLL, itself a restriction of linear logic. As a result, the
best way to present the type inference algorithm consists in first of all introducing
four auxiliary algorithms, each corresponding to a principle regulating the behavior of
the exponential connectives in linear logic. But before starting, a disclaimer: all algorithms
we will talk about have the ability to generate fresh variables. Strictly speaking, then, they
should take a counter (or anything similar) as a parameter, but we elide this for the sake of
simplicity. One fundamental property of many of the types produced in output by our inference
algorithm is the fact that index terms appearing in them are distinct function symbols applied
to the appropriate variables and to those from $\fiv$; in this case a type is said to be 
\emph{primitive for $\fiv$}. As an example, a primitive type for $\fiv=a,b$ is
$\NatU{f(a,b,c)}\marr{c<g(a,b)}\NatU{h(a,b,c)}$. An equational program $\ep$ is \emph{positively specified}
(respectively, \emph{negatively specified}) for a type $A$ if the only symbols appearing in $\ep$ but 
which are not specified by $\ep$ are those appearing in negative position (respectively,
in positive position) in $A$. Similarly definitions can be given for sequences of types.
\paragraph{Dereliction.}
Dereliction corresponds to the following principle: any duplicable object (say, of type $!A$)
can be made linear (of type $A$), that is to say $!A\rightarrow A$. In \dlpcf, being 
duplicable means having a modal type, which also contains a quantitative information, 
namely how many times the object can be duplicated, at most. Dereliction can be seen, 
as a consequence, simply as the principle $\mtyp{1}{A}\rightarrow A\isubst{0}$. Dereliction
is implicitly used in the $(App)$ rule: a function, which by definition is a duplicable object,
must be turned into a linear object before being applied to its argument. For every functional \PCF\ type
$T$, every index variable $a$ and every index context $\fiv$, one can build two linear 
\dlpcfv\ types $A$ and $B$ such that $A$ is primitive for $\fiv,a$
and $B$ is primitive for $\fiv$ and the two types are equivalent. Formally,
%\begin{lemma}[asdf]
  there is an algorithm $\algder$ such that $\algderp{\tpcfone}{\icontextone}{\ivarone}{\iconstraintone}{b}
  =((\mtypetwo,\mtypethree),\eqpone,\sscone)$ and where:
  \begin{varitemize}
  \item
    $\forget{\mtypeone}=\forget{\mtypetwo}=\tpcfone$;
  \item
    Whenever $\eqptwo\supseteq\eqpone$ is an equational program such that $\models^\eqptwo\sscone$,
    it holds that $\icontextone;\iconstraintone,\ivarone<1\vdash^\eqptwo\mtypetwo\teq\mtypethree$;
  \item
    $\mtypetwo$ is primitive for $\icontextone$, while $\mtypethree$ is primitive for $\icontextone,\ivarone$;
  \item
    $\eqpone$ is $b$-specified for $\mtypetwo$ and $\neg b$-specified for $\mtypethree$.
  \end{varitemize}
%\end{lemma}
The algorithm $\algder$ works by recursion on the \PCF\ type $\tpcfone$ and has thus linear complexity
in $|\tpcfone|$.
\paragraph{Contraction.}
Contraction is the principle according to which two copies of a duplicable object can actually be produced,
$!A\rightarrow !A,!A$. Contraction is used in binary rules like $(App)$ of $(If)$, in the form of the
operator $\uplus$. There is an algorithm $\algcontr$ such
that $\algcontrp{\tpcfone}{(\itermone,\itermtwo)}{\icontextone}{\ivarone}{\iconstraintone}{+}=
((\mtypetwo,\mtypethree,\mtypefour),\eqpone,\sscone)$ where:
\begin{varitemize}
\item
  $\forget{\mtypetwo}=\forget{\mtypethree}=\forget{\mtypefour}=\tpcfone$;
\item
  whenever $\eqptwo\supseteq\eqpone$ is an equational program such that $\models^\eqptwo\sscone$,
  it holds that $\icontextone;\iconstraintone\vdash^\eqptwo\qbang{\ivarone<\itermone+\itermtwo}
  {\mtypetwo}\teq(\qbang{\ivarone<\itermone}{\mtypefive})\uplus(\qbang{\ivarone<\itermtwo}{\mtypesix})$
  for some $\mtypefive$ and $\mtypesix$ such that
  $\icontextone;\iconstraintone,\ivarone<\itermone\vdash^\eqptwo\mtypefive\teq\mtypethree$
  and $\icontextone;\iconstraintone,\ivarone<\itermtwo\vdash^\eqptwo\mtypesix\teq\mtypefour$.
\item
  $\mtypetwo,\mtypethree,\mtypefour$ are all primitive for $\ivarone,\icontextone$;
\item
  $\eqpone$ is $b$-specified for $\mtypetwo$ and $\neg b$-specified for $\mtypethree,\mtypefour$.
\end{varitemize}
\paragraph{Weakening.}
Weakening means that duplicable objects are also erasable, even when the underlying index is $0$.
Weakening is useful in the $(Ax)$ rule, in particular. Concretely, weakening can be seen
as an algorithm $\algweak$ such that 
$\algweakp{\tpcfone}{\icontextone}{\ivarone}{b}=(\mtypetwo,\eqpone)$ where, as usual
\begin{varitemize}
\item
  $\forget{\mtypetwo}=\tpcfone$;
\item
  whenever $\eqptwo\supseteq\eqpone$ is an equational program, it holds that
  $\icontextone;\iconstraintone,\ivarone<0\vdash^\eqptwo\typetwo$;
\item
  $\mtypetwo$ is primitive for $\ivarone,\icontextone$;
\item
  $\eqpone$ is $b$-specified for $\mtypetwo$.
\end{varitemize}
Observe how no sets of constraints is produced in output by $\algweak$, contrarily to
$\algder$ and $\algcontr$.
\paragraph{Digging.}

\subsection{Soundness}
\label{sec:algo-snd}




\subsection{An Example}




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

